Detecting User Community in Sparse Domain via Cross-Graph Pairwise Learning

Cyberspace hosts abundant interactions between users and different kinds of objects, and their relations are often encapsulated as bipartite graphs. Detecting user community in such heterogeneous graphs is an essential task to uncover user information needs and to further enhance recommendation performance. While several main cyber domains carrying high-quality graphs, unfortunately, most others can be quite sparse. However, as users may appear in multiple domains (graphs), their high-quality activities in the main domains can supply community detection in the sparse ones, e.g., user behaviors on Google can help thousands of applications to locate his/her local community when s/he uses Google ID to login those applications. In this paper, our model, Pairwise Cross-graph Community Detection (PCCD), is proposed to cope with the sparse graph problem by involving external graph knowledge to learn user pairwise community closeness instead of detecting direct communities. Particularly in our model, to avoid taking excessive propagated information, a two-level filtering module is utilized to select the most informative connections through both community and node level filters. Subsequently, a Community Recurrent Unit (CRU) is designed to estimate pairwise user community closeness. Extensive experiments on two real-world graph datasets validate our model against several strong alternatives. Supplementary experiments also validate its robustness on graphs with varied sparsity scales.

==> content/deprecated.tex <==
\section{Experiment}
\subsection{Settings}
\subsubsection{Dataset}
We obtain two cross-domain datasets from Alibaba online scenario. The smaller dataset (Taobao\&Hema dataset) uses \textit{Taobao} as source domain and \textit{Hema} as target domain; While the larger dataset (Taobao\&Toutiao dataset) uses \textit{Taobao} as source domain and \textit{Toutiao} as target domain. \textit{Taobao} is the main shopping website holds by Alibaba Group, which occurs billions of user-item shopping behaviors each day. \textit{Toutiao} is a content recommendation system affiliated with \textit{Taobao} where users explore recommended feeds (articles or videos) based on their shopping behaviors. \textit{Hema} is a separate recipe recommendation application owned by Alibaba, in which users explore interesting recipes for cooking. Hence, the two datasets can be distinguished by scale and relevance between source and target domain. 

In this paper, `user' is regarded as shared nodes and `item'/ `feed'/ `recipe' are regarded as distinct nodes. Therefore, the two datasets can be converted to two cross-domain graphs where we aim to detect shared nodes (users) community structure on target graphs. The detailed statistic of both dataset is showed in Table \ref{tab:dataset}. In this paper, we sampled  80\% shared nodes as training nodes and the rest shared nodes testing nodes. To construct training data,  we sampled triplets solely constructed by training nodes. There are 203,123 triplets from Taobao \& Hema (T\&H) dataset and 2,072,905 triplets from Taobao \& Toutiao (T\&T) dataset. To construct validation and testing nodes, we sampled first node in the triplet from training nodes and the rest two nodes from testing nodes. There are 20,312 and 207,290 triplets in two datasets for testing and validation.

Given a triplet of shared nodes $<n_{i},n_{j},n_{k}>$, the label is $l \in \{0,0.5,1\}$ to measure the pairwise relationship $<n_{i},n_{j}>$ and $<n_{i},n_{k}>$. If the community relationship of $n_{j}>$ is closer than $n_{k}>$ towards $n_{i}>$, the label is 1; if the relationship is similar, the label is 0.5; otherwise the label is 0. Triplet labels are calculated via community detection methods on training nodes and whole nodes on the target domain graph for training, testing and validation respectively.
\begin{table}[h]
% \scriptsize

\small
\centering
\renewcommand{\tabcolsep}{1pt}
\renewcommand\arraystretch{0.5}
\begin{tabular}{ccccccc} 
  \toprule
\multirow{2}{*}{\textbf{Dataset}}& \multirow{2}{*}{\textbf{Shared   node}}&\multicolumn{2}{c}{\textbf{Source graph}}& \multicolumn{2}{c}{\textbf{Target graph}}\\ \cmidrule(c){3-6}
 &  &\textbf{Distinct node}& \textbf{Edge}&\textbf{Distinct node}& \textbf{Edge}\\ \midrule
T\&T& 105,702  & 492,549  & 17,352,482  & 26,133 & 881,721\\ 
T\&H& 1,029  & 1,543  & 1,161,293& 719   &147,266\\\bottomrule
\end{tabular}
% \vspace{-1em} 
\caption{Statistics of Two cross domain datasets}
\label{tab:dataset}
% \vspace{-1em} 
\end{table}  


\subsubsection{Parameter settings}
Based on empirical studies, we use mini-batch (size = 200) Adam optimizer to train our model with batch normalization and learning rate as 0.01. The default masked ratio on target domain inputs is 0.5. Distinct node embedding dimension is 128. Gradient clip value is 5.0. Community number for shared node is 50. Attentive vector is 64. Pairwise hidden layer dimension is 32. The community constraint weight is 0.01. We train the model for 10 epochs on each dataset in order to get a converged optimization. 
\subsubsection{Baseline and Metrics}
Six methods are selected from the state-of-the-art to comprehensively compare with our model performance of community detection on target domain graph. A random method and a well-designed iterative method are applied for comparison to make a total of eight baseline methods.

\begin{itemize}
    \item \textbf{random}: nodes are randomly assigned to a given number of communities.
    \item \textbf{Infomap} \cite{kheirkhahzadeh2016efficient}: A random walk based method to detect communities by minimizing the description length of walk paths\footnote{https://github.com/mapequation/infomap}.
    \item \textbf{DNR} \cite{yang2016modularity}: A novel nonlinear reconstruction method to detect communities by adopting deep neural networks on pairwise constraints among graph nodes\footnote{http://yangliang.github.io/code/}.
    \item \textbf{LSH} \cite{chamberlain2018real}: A random walk based method for community detection on large-scale graphs\footnote{https://github.com/melifluos/LSH-community-detection}.
    \item \textbf{node2vec} \cite{grover2016node2vec}: A skip-gram model to generate node emebeddings based on guided random walks on graphs. And K-means method calculates communities based on the generated embeddings.
    \item \textbf{BigClam} \cite{yang2013overlapping}: A non-negative matrix factorization method to detect overlapping communities on large scale graphs \footnote{https://github.com/snap-stanford/snap/}.
    \item \textbf{WMW} \cite{castrillo2017fast}: A fast heuristic method for hierarchical community detection inspired on agglomerative hierarchical clustering \footnote{https://github.com/eduarc/WMW}.
    \item \textbf{iterative}: node2vec method is used to generate shared node embeddings on source \& target domain graph separately first. After that, an iterative approach on source and target domain is designed. A linear Support vector machine method \cite{fan2008liblinear} is used on source domain\footnote{https://scikit-learn.org}, in which the input is source node embeddings and the output labels are communities generated from target domain. While in target domain, COP-Kmeans method \cite{wagstaff2001constrained} uses the top correctly predicted nodes from source domain as seed nodes, and returns shared node communities in a semi-supervised way\footnote{https://github.com/datamole-ai/active-semi-supervised-clustering}.
\end{itemize}

In this paper, when we regard label prediction as a classification task, Accuracy, Precision, Recall, F1-score, and Matthews Correlation Coefficient (MCC) are reported as evaluation metrics \cite{tsoumakas2007multi}. And when we regard it as a pairwise ranking task, Mean Reciprocal Rank (MRR), Normalized Discounted Cumulative Gain (NDCG), R-Precision (Rprec), Binary Preference (Bpref) and Mean Average Precision (MAP) are reported as evaluation metrics \cite{buckley2017evaluating}. 
\subsection{Results}
We evaluate our results from both classification and retrieval viewpoints. For each baseline method, we run it on three graphs including source graph, target graph and combined graph. For simplicity, we only report the best evaluation result among all three experiments.
\subsubsection{Classification Evaluation}

\begin{table}[h]
\scriptsize

\small
\centering
\renewcommand{\tabcolsep}{1.5pt}
\renewcommand\arraystretch{0.5}
\begin{tabular}{cccccc} 
  \toprule
 \multicolumn{6}{c}{\textbf{Taobao \& Toutiao Dataset}}\\
 \midrule 
 \textbf{Model}& \textbf{Accuracy} & \textbf{Precision}&\textbf{Recall}& \textbf{F1-score}& \textbf{MCC} \\ \midrule 
random &0.3337&0.3360&0.3331& 0.1788&-0.0008\\ 
Infomap &0.3625&0.5373&0.3621& 0.2567&0.0908\\ DNR&0.4383&0.5087&0.4381&0.4204&0.1817\\    
LSH &0.3992&0.4238&0.3992&0.4052&0.0993\\ node2vec  & 0.5072  &  0.5261 &0.5072&0.5124&0.2611\\   
BigClam &0.5580&0.5801&0.5580&0.5626&0.3412\\
WMW &0.6168&0.6330&0.6168&0.6205&0.4281\\
iterative& 0.5587  & 0.6207  &  0.5585  & 0.5605  &  0.3593 \\   
Our Model & \textbf{ 0.6524} & \textbf{0.6626 } & \textbf{0.6523 }& \textbf{0.6551 } &  \textbf{0.4808 }\\  \midrule 
\multicolumn{6}{c}{\textbf{Taobao \& Hema Dataset}}\\  \midrule 
random &0.3291&0.3174&0.3336&0.1699&0.0027\\ 
Infomap &0.3930&0.4198&0.3929&0.3988&0.0916\\
DNR&0.5273&0.5502&0.5273&0.5322&0.2957\\    
LSH &0.4180&0.4467&0.4184&0.4237&0.1309\\ node2vec&0.6015&0.6170&0.6015&0.6055&0.4045\\   
BigClam &0.5398&0.6128&0.5413&0.5383&0.3389\\
WMW &0.6682&0.6796&0.6682&0.6711&0.5041\\
iterative&0.6761&0.6887&0.6761&0.6788&0.5174\\ 
Our Model & \textbf{0.7740} & \textbf{0.7809} & \textbf{0.7739}& \textbf{0.7758} &  \textbf{0.6627}\\ \bottomrule
\end{tabular}
% \vspace{-1em} 
\caption{Classification evaluation result on pairwised cross-domain community detection}
\label{tab:classification-eval}
% \vspace{-1em} 
\end{table} 
 

\subsubsection{Retrieval Evaluation}

\begin{table}[h]
% \scriptsize

\small
\centering
% \renewcommand{\tabcolsep}{1pt}
\renewcommand\arraystretch{0.5}
\begin{tabular}{cccccc} 
  \toprule
 \multicolumn{6}{c}{\textbf{Taobao \& Toutiao Dataset}}\\
 \midrule 
 \textbf{Model}& \textbf{MRR} & \textbf{NDCG}&\textbf{Rprec}& \textbf{Bpref}& \textbf{MAP} \\ \midrule 
random &0.7815&0.8387&0.5631&   0.0065&0.7387\\ 
Infomap &0.7864&0.8423&0.5728&0.0073&0.7437\\ 
DNR&0.8101&0.8599&0.6203&0.0126&0.7686\\    
LSH &0.8020&0.8538&0.6040&0.0105&0.7599\\ 
node2vec  &0.8339&0.8774&0.6678&0.0218&0.7943  \\   
BigClam &0.8511&0.8901&0.7022&0.0324&0.8135\\
WMW &0.8702&0.9042&0.7404&0.0503&0.8353\\
iterative&0.8551&0.8931&0.7103&0.0356&0.8181\\   
Our Model & \textbf{0.8802} & \textbf{0.9116} & \textbf{0.7605}& \textbf{0.0634} &  \textbf{0.8470}\\  \midrule 
\multicolumn{6}{c}{\textbf{Taobao \& Hema Dataset}}\\  \midrule 
random &0.7739&0.8331&0.5479&  0.0055&0.7310\\ 
Infomap &0.7951&0.8488&0.5903&0.0089&0.7528\\
DNR&0.8391&0.8812&0.6781&0.0246&0.8000\\    
LSH &0.8021&0.8539&0.6041&0.0105&0.7600\\ 
node2vec  &0.8677&0.9023&0.7354&0.0475&0.8324\\   
BigClam &0.8475&0.8874&0.6950&0.0299&0.8095\\
WMW &0.8879&0.9173&0.7758&0.0757&0.8561\\
iterative&0.8908&0.9194&0.7815&0.0808&0.8595\\ 
Our Model & \textbf{0.9244} & \textbf{0.9442} & \textbf{0.8487}& \textbf{0.1753} &  \textbf{0.9005}\\ \bottomrule
\end{tabular}
% \vspace{-1em} 
\caption{Retrival evaluation result on pairwised cross-domain community detection}
\label{tab:retrieval-eval}
% \vspace{-1em} 
\end{table} 
 
\subsection{Model Exploration}

\subsubsection{Ablation Studies}
We iteratively removes each module of our model and see how the results changes. 

\begin{table}[h]
% \scriptsize

\small
\centering
\renewcommand{\tabcolsep}{1pt}
\renewcommand\arraystretch{0.5}
\begin{tabular}{p{3.5cm}ccccc} 
  \toprule
 \multicolumn{6}{c}{\textbf{Taobao \& Toutiao Dataset}}\\
 \midrule 
 \textbf{Model}& \textbf{Accuracy} & \textbf{Precision}&\textbf{Recall}& \textbf{F1-score}& \textbf{MCC} \\ \midrule 
--source graph community  &0.6263&0.6433&0.6264&0.6300&0.4432  \\   
--community propagation &0.5730&0.5903&0.5731&0.5769&0.3631\\
--item propagation &0.4793&0.5043&0.4793&0.4850	&0.2216\\
--community constraints&0.6319&0.6443&0.6319&0.6346&0.4507\\   
Joint & \textbf{0.6524} & \textbf{0.6626} & \textbf{0.6523}& \textbf{0.6551} &  \textbf{0.4808}\\  \midrule 
\multicolumn{6}{c}{\textbf{Taobao \& Hema Dataset}}\\  \midrule 
--source graph community  &0.7532&0.7611&0.7532&0.7548&0.6320  \\   
--community propagation &0.7178&0.7276&0.7179&0.7205&0.5782\\
--item propagation &0.5127&0.5352&0.5127&0.5175&0.2730\\
--community constraints&0.7312&0.7356&0.7309&0.7324&0.5976\\ 
Joint & \textbf{0.7740} & \textbf{0.7809} & \textbf{0.7739}& \textbf{0.7758} &  \textbf{0.6627}\\ \bottomrule
\end{tabular}
% \vspace{-1em} 
\caption{Ablation test on classification tasks to evaluate each module of our model. `--' means removing related modules from the model}
\label{tab:classification-ablation}
% \vspace{-1em} 
\end{table} 

\begin{table}[h]
% \scriptsize

\small
\centering
\renewcommand{\tabcolsep}{1.5pt}
\renewcommand\arraystretch{0.5}
\begin{tabular}{p{3.5cm}ccccc} 
  \toprule
 \multicolumn{6}{c}{\textbf{Taobao \& Toutiao Dataset}}\\
 \midrule 
\textbf{Model}& \textbf{MRR} & \textbf{NDCG}&\textbf{Rprec}& \textbf{Bpref}& \textbf{MAP} \\ \midrule 
--source graph community  &0.8729&0.9062&0.7458&0.0536&0.8384  \\   
--community propagation &0.8543&0.8924&0.7086&0.0349&0.8171\\
--item propagation &0.8277&0.8728&0.6554&0.0189&0.7875\\
--community constraints&0.8755&0.9081&0.7511&0.0569&0.8415\\   
Joint & \textbf{0.8802} & \textbf{0.9116} & \textbf{0.7605}& \textbf{0.0634} &  \textbf{0.8470}\\  \midrule 
\multicolumn{6}{c}{\textbf{Taobao \& Hema Dataset}}\\  \midrule 
--source graph community  &0.9179&0.9394&0.9179&0.1509&0.8924  \\   
--community propagation &0.9041&0.9292&0.8082&0.1099&0.8755\\
--item propagation &0.8363&0.8792&0.6726&0.0231&0.7970\\
--community constraints&0.9089&0.9328&0.8178&0.1228&0.8814\\ 
Joint & \textbf{0.9244} & \textbf{0.9442} & \textbf{0.8487}& \textbf{0.1753} &  \textbf{0.9005}\\ \bottomrule
\end{tabular}
% \vspace{-1em} 
\caption{Ablation test on retrieval tasks to evaluate each module of our model. `--' means removing related modules from the model}
\label{tab:retrieval-ablation}
% \vspace{-1em} 
\end{table} 


\subsubsection{Impact of graph sparseness} 
Define the graph sparseness for testing users.

Two figures to show how two metrics are changed with sparseness change.

\begin{figure}
	%\hspace*{-1cm} 
	\centering
	%%\subfloat[BLEU]{\includegraphics[width = 1.5in]{img/bleu.pdf}}  
	\subfloat[Toutiao]{\includegraphics[width = 1.8in]{img/toutiao.pdf}}
	\subfloat[Hema]{\includegraphics[width = 1.8in]{img/hema.pdf}} 
	\caption{Graph sparseness impact on model performance}
	%  \vspace{-2em}
	\label{fig:sparseness}
	%\vspace{-1.5em} 
\end{figure}

\subsubsection{Case Study}
Three real users community distribution on both graphs. And what user behaviors in the two domains. (for both dataset)

\begin{figure}  
% \advance\leftskip-1cm 
 \centering
 \includegraphics[width=1\columnwidth]{img/pipeline.png}
%  \vspace{-1em}
 \caption{A case study.}
 \label{fig:case}
\end{figure}
